Preconditioned Least-Squares Petrov-Galerkin Reduced Order Models

This paper introduces a methodology for improving the accuracy and efficiency of reduced order models (ROMs) constructed using the least-squares Petrov-Galerkin (LSPG) projection method through the introduction of preconditioning. Unlike prior related work, which focuses on preconditioning the linear systems arising within the ROM numerical solution procedure to improve linear solver performance, our approach leverages a preconditioning matrix directly within the LSPG minimization problem. Applying preconditioning in this way can improve ROM accuracy for several reasons. First, preconditioning the LSPG formulation changes the norm defining the residual minimization, which can improve the residual-based stability constant bounding the ROM solution's error. The incorporation of a preconditioner into the LSPG formulation can have the additional effect of scaling the components of the residual being minimized, which can be beneficial for problems with disparate scales. Importantly, we demonstrate that an 'ideal preconditioned' LSPG ROM (a ROM preconditioned with the inverse of the Jacobian of its corresponding full order model, or FOM) emulates projection of the FOM solution increment onto the reduced basis, a lower bound on the ROM solution error for a given reduced basis. By designing preconditioners that approximate the Jacobian inverse, a ROM whose error approaches this lower bound can be obtained. The proposed approach is evaluated in the predictive regime on several mechanical and thermo-mechanical problems within the Albany HPC code. We demonstrate numerically that the introduction of simple Jacobi, Gauss-Seidel and ILU preconditioners into the Proper Orthogonal Decomposition/LSPG formulation reduces significantly the ROM solution error, the reduced Jacobian condition number, the number of nonlinear iterations required to reach convergence, and the wall time.

==> alt_precond.tex <==


As shown in \textit{Remark 3} above, the introduction of a
preconditioner into the LSPG ROM formulation has the effect of
changing the norm in which the underlying ROM is optimal.  The best
case scenario corresponds to the case then ${\bm \Theta} = \I$,
which means $\Mk = \jkinv$.  Our objective here is to define
inexact, inexpensive-to-compute preconditioners for which $\Mk
\approx \jkinv$ so that ${\bm \Theta} \approx \I$.

%\irina{IKT: I could see that more accurate preconditioners would
%perform the best, since presumably $\Mk$ is closest to $\jkinv$ for
%those.  That would be consistent with the numerical results, I
%think.}{}

\irina{IKT: In our FY17 SAND report on the SPARC work, Jeff did some demonstrations in which 
the preconditioner was scaled by the element volumes.  Is that at all relevant for the Albany stuff?}{}

%\begin{itemize}
%\item Mention connection to $L^2$ weighted inner products - see equations (3.24) and (3.25)
%in FY17 SAND report.  \irina{IKT: it seems this is not relevant for
%Albany work.  Need to check with Payton and Jeff.}{}
%\item Discuss other preconditioners and arguments for their selection, e.g., ILU, Jacobi.
%\end{itemize}

In this work, 
we consider a range of preconditioners, including %we rely on the IFPACK suite of preconditioners within Trilinos \cite{ifpack-guide}.
%These IFPACK preconditioners include 
Jacobi, Gauss-Seidel, and symmetric Gauss-Seidel point relaxation preconditioning, and incomplete Cholesky (IC) and lower/upper (ILU) point incomplete factorizations.  The details of these preconditioning strategies are given in Section \ref{sec:precond_eval}.  
%Note that in the numerical results, the number following IC and ILU refers to the level of fill with the incomplete Cholesky and incomplete lower/upper preconditioners.
% TODO: include diagonal or not?
%In addition to the IFPACK provided preconditioners, two other modified approaches are also considered.  
%The first simply divides out every row $i$ of $\M{\lb}$, $\M{J}\M{\rb}$, and $\V{r}$ by the diagonal element of the FOM Jacobian $J_{ii}$ to obtain a better conditioned system.
%The second approach directly computes the solution $\V{\Delta x}$ of the FOM, \cref{eqn:FOM}, and then simply projects that FOM solution onto the ROM space to obtain the ROM solution $\V{\Delta \xi}$.
%Since we are actually solving the FOM system at every iteration instead of a modified ROM system as with the other approaches, the dominant source of error with this approach will be in the projection, i.e. how much the basis $\rb$ has been truncated, and we expect the errors with this approach to be very low.


==> galerkin.tex <==
Performing a classical Galerkin projection of \eqref{fomOver} onto
the reduced basis modes in the discrete $L^2$ inner product, we
obtain the following system
\begin{equation} \label{gal}
    \rb_M^T\res(\reference{\sol} + \rb\Galerkin{\reduced{\sol}}) = 0,
\end{equation}
where the approximate (Galerkin) solution is $\Galerkin{\approximate{\sol}}\defeq\reference{\sol} +
\rb_M\Galerkin{\reduced{\sol}}$. Assuming \eqref{gal} is solved using the classical
Newton algorithm, the reduced Newton iterations take the form:
\begin{gather} \label{galitne}
    \Galerkin{\jac}\newton{k} \delta\Galerkin{\reduced{\sol}}  =
    -\Galerkin{\res}\newton{k},
    \quad k=1,\ldots,\Galerkin{K},\\
    %
    \Galerkin{\reduced{\sol}} = \Galerkin{\reduced{\sol}} + \lengthk\delta\Galerkin{\reduced{\sol}},\\
	\Galerkin{\approximate{\sol}} = \reference{\sol} + \rb_M\Galerkin{\reduced{\sol}}, \\
\end{gather}
where $\Galerkin{\jac}\newton{k} = {\rb_M}^T \jac\newton{k}\rb$,
$\Galerkin{\res}\newton{k} = {\rb_M}^T \res\newton{k}$,
and $\Galerkin{K}$ is the number of Newton iterations.

Despite its popularity, the Galerkin approach to model reduction is
known to have some disadvantages when applied to certain classes of problems, e.g., compressible flow. 
In particular, %it is well-known that 
reduced order models
constructed using the POD/Galerkin method may lack in general an
\textit{a priori} stability guarantee. Thus, it can happen that a
POD/Galerkin constructed for a stable full order model exhibits a
non-physical instability, which can lead to practical limitations of
the ROM: as demonstrated in \cite{buithanh, kalashSAND, kalashACM,
baronekalash, baroneJCP}, a %compressible fluid POD/Galerkin 
ROM might be stable for a given number of modes, but unstable for other
choices of basis dimension. \\

%With a Galerkin projection approach, the left basis $\lb$ of
%\cref{ROM:Newton} is chosen to be equal to the reduced basis $\rb$.

%\irina{IKT question: are we going to show results with Galerkin
%projection?  If not, take out this section.}{}


==> ideal_precond.tex <==

%\begin{itemize}
%\item Mention connection to projection of true FOM solution increment.
%\item Mention that ideal preconditioner will lead to optimal $l^2$ projection of the solution increment
%onto the basis.  See FY17 and FY18 SAND reports \cite{fy17_sand,
%fy18_sand}.
%\end{itemize}

\irina{IKT TODO: need to simplify this discussion.}{}

We first discuss the specific case of an ideal preconditioned LSPG
ROM, namely a ROM in which $\Mk:= \jkinv$ in \eqref{lspgit_prec}.

We begin by defining the so-called ``projected solution increment'',
which determines the upper limit on the ROM accuracy.  If
$\delta\sol\newton{k}$ is the solution increment computed by the FOM at time
step $k$ (from \eqref{fom_newton}), then
\begin{equation} \label{eq:projsol3}
    \delta\approximate{\sol}\newton{k} = \rb_M \left( \rb^T \rb \right)^{-1} \rb^T \delta\sol\newton{k}
\end{equation}
is the approximated solution increment.

It is straightforward to show that the projected solution increment
given by \eqref{eq:projsol3} is equivalent to what would be produced
by a preconditioned LSPG ROM using an exact preconditioner
\begin{equation} \label{exact_prec}
\Mk= \jkinv.
\end{equation}
Substituting \eqref{exact_prec} into \eqref{lspgitne_prec} reduces
these normal equations to
\begin{equation} \label{lspgitne_ideal_prec}
    \rb_M^T\rb\delta\PrecondPetrovGalerkin{\reduced{\sol}}\newton{k}  = -\rb^T\jkinv\rk, \quad k=1,\ldots,\PrecondPetrovGalerkin{K}
\;.
\end{equation}
Recognizing that the right-hand side of \eqref{lspgitne_ideal_prec}
contains the FOM solution increment $\delta\sol\newton{k} = -\jkinv\rk$,
\eqref{lspgitne_ideal_prec} is equivalent to
\begin{equation} \label{lspgitne_ideal_prec2}
    \delta\PrecondPetrovGalerkin{\reduced{\sol}}\newton{k}  = (\rb_M^T\rb)^{-1}\rb^T\delta\sol\newton{k}, \quad
    k=1,\ldots,\PrecondPetrovGalerkin{K} \;,
\end{equation}
so that, from \eqref{eq:subspace}, is given by \eqref{eq:projsol3}. \\ 
%The projected solution increment \eqref{eq:projsol3} can then be 
%calculated using \eqref{lspgitne_ideal_prec2}. \\

\noindent {\bf \textit{Remark 2.}} Remark that
\eqref{lspgitne_ideal_prec2} defines the normal equations for the
following minimization problem
\begin{equation} \label{opt_ideal_precond}
    \delta\PrecondPetrovGalerkin{\reduced{\sol}}\newton{k} \in \arg
\min_{\dummySol\in\RR{\nrb}}\|\rb_M\dummySol - \delta\sol\newton{k}\|_2^2
\end{equation}
That is, the use of the ideal preconditioner $\Mk = \jkinv$ leads to an $l^2$-optimal projection of the solution increment
$\delta\sol\newton{k}$ onto the reduced basis $\rb_M$. \\

%\irina{IKT: very basic, possibly dumb question: why is the $l^2$
%norm the ``best'' norm?  Presumably the stability constants are the
%best?}{}

\noindent {\bf \textit{Remark 3.}} Comparing
\eqref{opt_ideal_precond} with \eqref{opt}, we can see that the idea
preconditioner leads to search directions $\delta\PrecondPetrovGalerkin{\reduced{\sol}}\newton{k}$ that are
optimal in the sense of \eqref{opt} with ${\bm \Theta} = \I$. For
the more general case of an arbitrary preconditioner $\Mk$, it is
straight-forward to see that \eqref{lspgit_prec}
is equivalent to \eqref{opt} with ${\bm \Theta} = (\Mk \jk)^{T} \Mk \jk$. \\

\noindent {\bf \textit{Remark 4.}} There is an additional benefit of
introducing a preconditioner into the LSPG formulation \eqref{lspg}.
Remark that, with the addition of the preconditioner $\M$, the
least-squares optimization problem \eqref{lspg} takes the form:
\begin{equation} \label{precond_lspg}
    \PrecondPetrovGalerkin{\reduced{\sol}} \in \arg\min_{\dummySol\in\RR{\nrb}}\|\M \res(\reference{\sol} +
    \rb_M\dummySol)\|_2^2.
\end{equation}
It has been observed \cite{kyle} that minimizing the raw
(unweighted) residual $\res$ can be problematic for systems of PDEs
where different variables have drastically different magnitudes,
which happens frequently in various applications where dimensional
equations are employed.  Residual components corresponding to
certain variables can be very large compared to the residual
components corresponding to other variables, thereby biasing the
minimization procedure.  As shown in \cite{kyle}, scaling the ROM
residual to get all the equations to be roughly the same order of
magnitude can remedy this problem.  Remark that the introduction of
a preconditioner $\M$ can have the same effect.  \\

\irina{IKT FIXME: we should discuss the implication of the norm in
which the minimization is done on the error constants, but I'm not
sure what to cite for this and which norm has the lowest error
bounds.  I'm guessing the error constants depend on the norm and the
$l^2$ norm is the best one? }{}

\irina{IKT FIXME:  Note that Galerkin projection can be recovered by
setting $\Mksqr = \jkinv$, though that is not always a norm (as we
know). Not sure what to make of this...  Supposedly Jeff had some
notes showing that preconditioned LSPG is equivalent to Galerkin -
may be worth digging this up.}{}


\irina{IKT comment from Kevin: Cite the error analysis in other
papers and state that the preconditioner should yield a smaller
stability constant, which in turn yields smaller error bounds - can
be written as a remark instead of Discussion subsection.}{}

\irina{IKT: I'm not sure exactly what papers Kevin has in mind here
to cite. Payton, Jeff: do you?}{}


==> projection.tex <==

Here, we consider two ways to compute a unique solution $\reduced{\sol}$ within a projection-based
model reduction framework:
Galerkin projection and Least-Squares Petrov--Galerkin (LSPG)
projection. \\


\noindent \textbf{Galerkin projection.} \input{galerkin}

\noindent \textbf{Least-squares Petrov--Galerkin (LSPG) projection.}
\input{lspg}


